ThinkLess: A Training-Free Inference-Efficient Method for Reducing Reasoning Redundancy

While Chain-of-Thought (CoT) prompting improves reasoning in large language models (LLMs), the excessive length of reasoning tokens increases latency and KV cache memory usage, and may even truncate final answers under context limits. We propose ThinkLess, an inference-efficient framework that terminates reasoning generation early and maintains output quality without modifying the model. Atttention analysis reveals that answer tokens focus minimally on earlier reasoning steps and primarily attend to the reasoning terminator token, due to information migration under causal masking. Building on this insight, ThinkLess inserts the terminator token at earlier positions to skip redundant reasoning while preserving the underlying knowledge transfer. To prevent format discruption casued by early termination, ThinkLess employs a lightweight post-regulation mechanism, relying on the model's natural instruction-following ability to produce well-structured answers. Without fine-tuning or auxiliary data, ThinkLess achieves comparable accuracy to full-length CoT decoding while greatly reducing decoding time and memory consumption.

==> tables/document.tex <==
\begin{table*}[t]
\centering
\caption{}
\label{}
\resizebox{\textwidth}{!}{
    \begin{tabular}{lcccc|cccc|cccc|cccc|cccc}
        \toprule
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{GSM8K}} & \multicolumn{4}{c}{\textbf{MMLU}} & \multicolumn{4}{c}{\textbf{GPQA}} & \multicolumn{4}{c}{\textbf{BBH}} & \multicolumn{4}{c}{\textbf{AVG.}} \\
        \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17} \cmidrule(lr){18-21}
        & \textbf{Acc↑} & \textbf{Time↓} & \textbf{Peak↓} & \textbf{Dep↓} & \textbf{Acc↑} & \textbf{Time↓} & \textbf{Peak↓} & \textbf{Dep↓} & \textbf{Acc↑} & \textbf{Time↓} & \textbf{Peak↓} & \textbf{Dep↓} & \textbf{Acc↑} & \textbf{Time↓} & \textbf{Peak↓} & \textbf{Dep↓} & \textbf{Acc↑} & \textbf{Time↓} & \textbf{Peak↓} & \textbf{Dep↓} \\
        \midrule
        \rowcolor{gray!20}\multicolumn{21}{c}{\textit{Qwen2.5-7B Series}} \\
        \midrule
        CoT & 27.75 & 1.66 & 513 & 0.1M & 66.50 & 1.77 & 649 & 0.2M & 26.76 & 0.60 & 968 & 0.5M & 65.45 & 0.68 & 570 & 0.1M & 46.62 & 1.18 & 675 & 0.2M \\
        Distill-R1 & 81.88 & 5.60 & 844 & 1.1M & 28.24 & 14.31 & 2483 & 7.5M & 10.10 & 8.01 & 6718 & 31M & 57.78 & 5.53 & 1967 & 6.0M & 44.50 & 8.36 & 3003 & 11.3M \\
        \midrule
        Vanilla & 90.90 & 11.83 & 2086 & 3.9M & 59.98 & 20.61 & 3417 & 10M & 30.81 & 10.76 & 8055 & 39M & 69.90 & 11.50 & 3786 & 13M & 62.90 & 13.68 & 4336 & 16.6M \\
        + H2O & \underline{89.92} & 22.19 & \textbf{640} & \underline{1.2M} & \underline{59.69} & 29.02 & {1024} & 3.2M & 24.75 & 15.61 & \underline{1200} & \underline{9.8M} & \underline{70.10} & 15.61 & \textbf{1024} & \underline{3.5M} & \underline{61.12} & 20.61 & \textbf{972} & \underline{4.4M} \\
        + SepLLM & 30.40 & 53.52 & 1024 & 6.9M & 10.81 & 53.45 & 1024 & 9.0M & 0.00 & 11.65 & \textbf{1024} & 10M & 8.08 & 26.64 & 1024 & 9.4M & 12.32 & 36.32 & \underline{1024} & 8.9M \\
        AnLLM & 78.39 & 15.26 & 789 & 1.6M & 54.63 & 14.13 & \underline{875} & \underline{2.0M} & 19.70 & 9.14 & 3401 & 11M & 54.95 & 10.04 & 1303 & 3.8M & 51.92 & 12.14 & 1592 & 4.6M \\
        \midrule
        Ours (tho.) & \textbf{90.14} & \textbf{11.46} & \underline{676} & \textbf{1.0M} & \textbf{60.47} & \textbf{13.09} & {944} & \textbf{1.9M} & \textbf{30.30} & \underline{8.41} &{2385} & \textbf{9.3M} & \textbf{70.30} & \textbf{7.71} & \underline{1151} & \textbf{2.7M} & \textbf{62.80} & \textbf{10.17} & {1289} & \textbf{3.7M} \\
        Ours (token) & 87.11 & \underline{11.48} & {1038} & 1.5M & 57.35 & \underline{13.80} & \textbf{489} & 3.5M & \underline{28.28} & \textbf{8.26} & {3940} & 18M & 62.83 & \underline{8.95} & {1884} & 5.6M & 58.89 & \underline{10.62} & {1838} & 7.2M \\
        \midrule
        \rowcolor{gray!20}\multicolumn{21}{c}{\textit{Llama3.1-8B Series}} \\
        \midrule
        CoT & 85.14 & 2.15 & 550 & 0.2M & 65.82 & 2.39 & 736 & 0.3M & 24.75 & 0.96 & 1231 & 0.9M & 66.46 & 0.93 & 642 & 0.2M & 60.54 & 1.61 & 790 & 0.4M \\
        Distill-R1 & 73.62 & 2.58 & 395 & 0.1M & 22.01 & 2.97 & 582 & 0.8M & 20.20 & 5.24 & 3972 & 16M & 37.58 & 0.83 & 380 & 0.2M & 38.35 & 2.91 & 1332 & 4.4M \\
        \midrule
        Vanilla & 91.43 & 12.06 & 1986 & 3.0M & 69.62 & 14.82 & 2883 & 6.9M & 40.91 & 7.98 & 6622 & 26M & 83.03 & 6.80 & 2793 & 5.9M & 71.25 & 10.42 & 3571 & 10.5M \\
        + H2O & \textbf{90.45} & 20.23 & {640} & \underline{1.0M} & \textbf{65.92} & 27.11 & \underline{736} & 1.8M & 31.81 & 12.55 & {1536} & 7.9M & \underline{78.99} & 11.43 & {1024} & 2.1M & \underline{66.79} & 17.83 & \underline{984} & 3.2M \\
        + SepLLM & 26.25 & 50.05 & {1024} & 5.8M & 25.12 & 50.11 & {1024} & 7.5M & 2.53 & 12.62 & \underline{1024} & 10M & 14.55 & 27.14 & {1024} & 8.5M & 17.11 & 34.98 & {1024} & 8.0M \\
        AnLLM & 77.33 & 17.92 & \textbf{589} & 1.1M & 58.62 & 16.53 & \textbf{589} & \textbf{1.2M} & 31.31 & 7.19 & \textbf{838} & \textbf{3.7M} & 68.89 & 9.79 & \textbf{621} & \textbf{1.6M} & 59.04 & 12.86 & \textbf{659} & \textbf{1.9M} \\
        \midrule
        Ours (tho.) & \underline{88.25} & \textbf{12.65} & \underline{629} & \textbf{0.9M} & \underline{63.39} & \textbf{14.88} & {882} & \underline{1.8M} & \textbf{36.36} & \textbf{6.38} & {1796} & \underline{6.4M} & \textbf{79.39} & \underline{7.46} & \underline{911} & \underline{1.9M} & \textbf{66.85} & \textbf{10.34} & {1055} & \underline{2.7M} \\
        Ours (token) & 85.52 & \underline{13.87} & {1104} & 1.7M & 61.05 & \underline{15.85} & {1538} & 3.3M & \underline{31.82} & \underline{6.94} & {3150} & 12M & 74.14 & \textbf{7.43} & {1512} & 2.9M & 63.13 & \underline{11.02} & {1826} & 4.8M \\
        \bottomrule
    \end{tabular}
}
\end{table*}

==> tables/full_dataset_1.tex <==
\begin{table*}[t]
    \renewcommand\arraystretch{1.3}
    \setlength{\tabcolsep}{5pt}
    \centering
    \small
    \begin{tabularx}{\textwidth}{c|c|XXX|XXX|XXX|XXX|XXX}
        \bottomrule
        \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Type}} &
        \multicolumn{3}{c|}{\textbf{GSM8k}} &
        \multicolumn{3}{c|}{\textbf{GPQA}} &
        \multicolumn{3}{c|}{\textbf{BBH}} &
        \multicolumn{3}{c|}{\textbf{MMLU}} &
        \multicolumn{3}{c}{\textbf{Math500}} \\
        % \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14} \cmidrule(lr){15-17}
        & & \textbf{RL} & \textbf{TL} & \textbf{Acc} &
        \textbf{RL} & \textbf{TL} & \textbf{Acc} &
        \textbf{RL} & \textbf{TL} & \textbf{Acc} &
        \textbf{RL} & \textbf{TL} & \textbf{Acc} &
        \textbf{RL} & \textbf{TL} & \textbf{Acc} \\
        \hline
        \multirow{2}{*}{\textbf{qwen-base}} &
        \textbf{reason} & & & & & & & & & & & & & & & \\
        & \textbf{no reason} & & & & & & & & & & & & & & & \\
        \hline
        \multirow{2}{*}{\textbf{qwen-r1-7b}} &
        \textbf{reason} & & & & & & & & & & & & & & & \\
        & \textbf{no reason} & & & & & & & & & & & & & & & \\
        \hline
        \multirow{2}{*}{\textbf{qwen-r1-14b}} &
        \textbf{reason} & & & & & & & & & & & & & & & \\
        & \textbf{no reason} & & & & & & & & & & & & & & & \\
        \hline
        \multirow{2}{*}{\textbf{llama-base}} &
        \textbf{reason} & & & & & & & & & & & & & & & \\
        & \textbf{no reason} & & & & & & & & & & & & & & & \\
        \hline
        \multirow{2}{*}{\textbf{llama-r1-8b}} &
        \textbf{reason} & & & & & & & & & & & & & & & \\
        & \textbf{no reason} & & & & & & & & & & & & & & & \\
        \bottomrule
    \end{tabularx}
    \caption{Performance comparison of different models on reasoning datasets with and without reasoning (RL) and token length (TL).}
    \label{tab:performance_comparison}
\end{table*}

==> tables/full_dataset_table.tex <==

\begin{table*}[t]
\renewcommand\arraystretch{1.3}
\setlength{\tabcolsep}{4pt}
\centering
\small
% \begin{tabular}{\textwidth}{p{1.4cm}p{2cm}cccccc}
\begin{tabularx}{\textwidth}{c|c|ccc|ccc}
\bottomrule
    \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{type}} & \multicolumn{3}{c|}{\textbf{DS-R1-Distill-Qwen-7B}} & \multicolumn{3}{c}{\textbf{DS-R1-Distill-Llama-8B}} \\
    % \cmidrule(lr){3-5} \cmidrule(lr){6-8}
    & & \textbf{Acc} & \textbf{R.Len} & \textbf{T.Len} & \textbf{Acc} & \textbf{R.Len} & \textbf{T.Len} \\
    \hline
    \multirow{2}{*}{GSM8k} & full reasoning & 88.17 & 1.00 & 1.00 & 79.38 & 1.00 & 1.00 \\
    & no reasoning & 87.79 & 0.00 & 0.64 & 79.76 & 0.01 & 0.64 \\
    \hline
    \multirow{2}{*}{GPQA} & full reasoning & 30.81 & 1.00 & 1.00 & 25.76 & 1.00 & 1.00 \\
    & no reasoning & 30.81 & 0.00 & 0.16 & 30.30 & 0.00 & 0.13 \\
    \hline
    \multirow{2}{*}{BBH} & full reasoning & 69.29 & 1.00 & 1.00 & 71.92 & 1.00 & 1.00 \\
    & no reasoning & 61.82 & 0.01 & 0.45 & 65.45 & 0.01 & 0.37 \\
    \hline
    \multirow{2}{*}{MMLU} & full reasoning & 60.86 & 1.00 & 1.00 & 64.26 & 1.00 & 1.00 \\
    & no reasoning & 54.04 & 0.00 & 0.25 & 57.45 & 0.00 & 0.22 \\
    \hline
    \multirow{2}{*}{MATH 500} & full reasoning & 81.00 & 1.00 & 1.00 & 76.80 & 1.00 & 1.00 \\
    & no reasoning & 75.40 & 0.00 & 0.25 & 71.60 & 0.00 & 0.22 \\
\toprule
\end{tabularx}
\caption{Evaluation of five reasoning datasets, focusing on complex scientific, mathematical, and logical tasks. The maximum sequence length is set to 8192, and the lengths are presented in a ratio format.}
\label{tab:full_set_eval}
\end{table*}

